OpenKinoAI: An Open Source Framework for Intelligent Cinematography and Editing of Live Performances

OpenKinoAI is an open source framework for post-production of ultra high definition video which makes it possible to emulate professional multiclip editing techniques for the case of single camera recordings. OpenKinoAI includes tools for uploading raw video footage of live performances on a remote web server, detecting, tracking and recognizing the performers in the original material, reframing the raw video into a large choice of cinematographic rushes, editing the rushes into movies, and annotating rushes and movies for documentation purposes. OpenKinoAI is made available to promote research in multiclip video editing of ultra high definition video, and to allow performing artists and companies to use this research for archiving, documenting and sharing their work online in an innovative fashion.

==> OpenKinoAI Overview/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> OpenKinoAI Overview/stateoftheart.tex <==


%Chercher à étudier la représentation théâtrale, c’est tenter de saisir l’éphémère : tous les pédagogues et chercheur.e.s en arts de la scène en ont fait l’expérience, analyser une représentation qui a déjà eu lieu s’apparente nécessairement à un processus de reconstruction subjectif et fragmentaire. Le recours à la captation vidéo ne permet pas de résoudre l’ensemble des difficultés posées par l’étude d’un objet qui n’existe plus : selon l’angle choisi, une partie du spectacle peut échapper à l’oeil de la caméra, le son est souvent médiocre et l’expérience face à l’écran rend peu compte de celle du spectateur en salle.

%Cette difficulté est d’autant plus grande lorsqu’on choisit de s’intéresser aux processus de création, c’est-à-dire à la façon dont émerge l’acte théâtral en répétitions, dans la lignée des rehearsal studies (1). Si de très nombreuses compagnies théâtrales utilisent depuis longtemps la vidéo pour filmer leurs répétitions, le plus souvent dans le but de créer une « mémoire » de la compagnie, d’enregistrer ces moments fugaces et souvent décrits comme « magiques » que sont les répétitions, force est de constater que ces heures de captations sont rarement « traitées » et s’entassaient hier dans des cartons (en format dv) ou s’accumulent aujourd’hui sur des disques durs externes.

%Reprenant un dispositif qui avait déjà été expérimenté au cours d’un projet précédent, Spectacle en ligne (3), nous avons placé une unique caméra au milieu de l’orchestre, une position qui est également privilégiée par le metteur en scène pour observer les répétitions. Nous avons suivi en cela une proposition ingénieuse de Jean-Luc Godard (4) : « Pourquoi les gens de théâtre n’ont-ils jamais envie de filmer leurs spectacles pour les garder comme archives ? (…) Ce serait très simple : la caméra au milieu de l’orchestre avec un objectif moyen – mais pas le zoom, qui donnerait déjà lieu à une interprétation ».

%Ce « point de vue du metteur en scène » présente plusieurs avantages théoriques et pratiques. D’une part, c’est le point de vue le plus adapté à la projection des films des spectacles dans la même salle. D’autre part, c’est le point de vue le plus proche des acteurs, et le seul qui permette de saisir le jeu des regards entre les acteurs et la salle. Enfin, c’est également le point de vue pour lequel les éclairages sont mis au point, ce qui nous permet de filmer sans modifier ces éclairages. Ce dernier point reste difficile à réaliser en pratique, surtout lorsque les éclairages varient brusquement, mais cela nous paraît important de respecter les choix de mise en scène, ce qui n’est possible que de ce seul point de vue.

%Comme le souligne justement Pascal Bouchez (5), une problématique particulière à la captation vidéo, c’est l’opposition entre le traitement parallèle de l’information au théâtre (le spectateur voit l’ensemble des acteurs et perçoit globalement la scène), et le traitement séquentiel de cette même information au cinéma ou à la télévision (le spectateur ne voit que les acteurs choisis par le réalisateur et perçoit donc de façon séquentielle la scène à travers une suite d’images). Ainsi, le suivi séquentiel des dialogues peut être problématique lorsque ceux-ci font intervenir trois acteurs éloignés. Un plan fixe des trois acteurs ne permet pas facilement au spectateur de se repérer à l’écran comme il le ferait face à la scène. Une série de gros plans peut être utilisée pour diriger l’attention du spectateur. Il faut donc bien comprendre le système cognitif de l’attention et son fonctionnement dans les deux situations différentes de la scène et de l’écran.

%Les techniques classiques du cinéma permettent en principe de résoudre ces différents problèmes, par une transposition entre les langages dramatique et cinématographique. Mais dans les conditions du direct, le réalisateur est de plus en plus démuni au fur et à mesure que croît le volume spatial de la scène. Comme l’écrit Pascal Bouchez, “tout se joue en direct, si vite que les plans dont la création nécessiteraient de nombreuses répétitions et une longue préparation au cinéma – sont impossibles au théâtre”.

 %Le projet de recherche Kino Ai aborde précisément cette question grâce à des techniques d’intelligence artificielle qui proposent automatiquement des solutions de cadrage et de montage montrant les actions scéniques et leur enchainement : les données extraites des heures filmées peuvent ainsi s’adapter aux besoins exprimés soit par les professionnels du spectacle, soit par les enseignants et les chercheurs (archivage pour la compagnie, communication auprès des diffuseurs, documentation pour la pédagogie et/ou la recherche).

%On peut remarquer que cette méthode de recadrage en post-production est une option technique et artistique nouvelle, décrite par Walter Murch sous le nom de montage vertical (6), et qui permet de contrôler le « zoom de l’interprétation » dont parlait Jean-Luc Godard en post-production. Cette technique est particulière fastidieuse pour les monteurs, mais se prête en revanche très bien au traitement informatique.

%A partir d’une captation unique, nous proposons ainsi des solutions de montage multiples, destinés à visualiser la captation selon plusieurs lectures possibles. Notre approche tire parti du fait que tous les rushes peuvent être virtuellement disponibles. Dans un autre contexte, Francis Ford Coppola a utilisé cette possibilité pour intervenir en direct sur le montage de son film Twixt lors de projections en festivals (7).

%En suivant ce principe, nous calculons plusieurs cadres mettant en avant les différents aspects de la représentation théâtrale : décors et mouvements d’acteurs en plan large ; codes de proximités entre les acteurs en plan moyen ; langage verbal et non verbal en plan rapproché. Chaque série de plans ainsi recadrés peut être organisée en temps réel en un montage dédié au point de vue choisi. Cette technique permet l’exploration de la représentation sous ses différents aspects.

%-----------------------------------------
\section{State of the art}
Previous work in intelligent cinematography and editing is numerous.

Some previous work has been devoted to generating cinematographic rushes from wide-screen video in various contexts, including meetings \cite{???}, courses \cite{???}, video conferences \cite{???} and live performances \cite{Gandhi2014,Kumar2017}.


The problem of creating a multi-view edited video from limited
input camera views has been considered previously in very specialized
scenarios. The Virtual Videography system \cite{Heck2007} used virtual
PTZ to simulate multiple cameras from a lecture video. The
MSLRCS \cite{Zhang2005} and AutoAuditorium \cite{Bianchi2004} systems 
use a small set of fixed views including input of presentation slides. These systems achieve full automation, albeit at the expense of allowing for creativity
and human input in the editing process. They are also limited
to working in the more constrained environment of usually a
single presenter in front of a chalkboard or a slide screen. Extending
to the richer environment of multiple actors in more complex
stagings would be challenging, especially as it requires a richer set
of shot types to be generated. In contrast, our system addresses
only the rush generation aspect, but can generate a rich range of
shot types from more complex scenarios including multiple actors.

Remarkably little work as been devoted specifically to the problem
of optimizing the composition of a virtual PTZ camera in postproduction.
Recent work has focused more on providing interactive
control of the virtual PTZ camera in real time \cite{Gaddam2014a,Gaddam2014b}. A method for automatic editing of basketball games was also proposed
by Carr et al. \cite{Carr2013} employing both robotic and virtual PTZ cameras.
The robotic camera follows the centroid of the detected players and
then a virtual camera is employed to crop subregions of the obtained
images to compensate for motor errors. Because they are
targeting online applications, their method makes decisions in near
real time (with a small delay), which can lead to sub-optimal solutions.
To the best of our knowledge, our technique provides the first
general solution to the problem for offline computation of a virtual
pan-tilt-zoom camera shot given a list of visual targets over the entire
duration of a recorded performance.

The question of a computational model to describe “good” camera
movements, particularly in terms of subwindows of video, has been
considered by work in video stabilization. While most previous work in
video stablization simply aim to remove jitter, Re-Cinematography
\cite{Gleicher2008} formalized cinematic principles in terms of movement in the
frame for computation. Grundmann et al. then showed that this
can be formulated in an optimization framework \cite{Grundmann2011}. We build on this computational formulation of camera movement, extending it to the
problem of multiple rush generation.

Several frameworks for automatically cropping sub-clips from a
panoramic video and editing them together into a movie in realtime
has been proposed for the case of sports events \cite{Daniyal2011,Schreer2013}. Operating in real-time limits the capability of that system to tracking of
simple targets. Because we are focusing on post-production, rather
than live broadcast, we are able to perform tracking and recognition
of multiple actors even in complex cases, which makes our method
more generally applicable to rich cultural heritage content. Furthermore,
our method can be used to generate arbitrary shot compositions.

Pano2Vid \cite{Su2016} is a new computer vision problem where the task is to  automatically control the pose and motion of a virtual normal-field-of-view (NFOV) camera within an input 360° video. Camera control must be optimized to produce video that could conceivably have been captured by a human observer equipped with a real NFOV camera. 

Using computer vision to control cameras and create full-edited
movies is not a new idea. Pinhanez and Bobick \cite{Pinhanez1997} have investigated the use of low-level motion tracking to control TV cameras  but their method is limited to closed-world domains (exemplified
by cooking shows) and requires extensive domain-specific
knowledge. 

Our method assumes a pre-processing stage, where actors are tracked
and the location of their heads and floor projections are recovered
in each frame of the input video. We use actor poses detected by the OpenPose software as an input \cite{OpenPose}. Kinoai includes software for automatically linking those poses into tracklets  and a graphical user interface for labeling and naming tracklets. 
 
\RR{Include more references for tracking and naming actors}

\RR{Include more references for cropping panoramic video}



Tedial  proposes a technology called SmartLive For Live Events And Production
\footnote{Tedial behind the play, 2019, \url{https://www.tedial.com}}.

Pixellot’s [4] patented technology streamlines the production workflow by deploying an unmanned multi-camera system in a single fixed rig \footnote{Pixellot Automatic Production,» 2019 \url{https://www.pixellot.tv}}.

Seervision \footnote{\url{https://www.seervision.com}} has analysed the motion sequences of cameramen in various scenarios and converted them into video analysis algorithms for real-time object recognition and scene segmentation. 


Other previous  work has investigated automatic film editing of multi-camera live performances\cite{Wright2018} and dialogue scenes \cite{Leake2017}.

Automated video capture and analysis of live theatre was the focus of the "spectacle en ligne(s)" experimental system, which was used to create an online dataset of 300 hours of rehearsals \cite{Ronfard2015}. 

To the best of our knowledge, there is no existing  open source programming environment for consolidating this preview work together. Kino AI aims to provide such an environment. 


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> stateoftheart.tex <==


%Chercher à étudier la représentation théâtrale, c’est tenter de saisir l’éphémère : tous les pédagogues et chercheur.e.s en arts de la scène en ont fait l’expérience, analyser une représentation qui a déjà eu lieu s’apparente nécessairement à un processus de reconstruction subjectif et fragmentaire. Le recours à la captation vidéo ne permet pas de résoudre l’ensemble des difficultés posées par l’étude d’un objet qui n’existe plus : selon l’angle choisi, une partie du spectacle peut échapper à l’oeil de la caméra, le son est souvent médiocre et l’expérience face à l’écran rend peu compte de celle du spectateur en salle.

%Cette difficulté est d’autant plus grande lorsqu’on choisit de s’intéresser aux processus de création, c’est-à-dire à la façon dont émerge l’acte théâtral en répétitions, dans la lignée des rehearsal studies (1). Si de très nombreuses compagnies théâtrales utilisent depuis longtemps la vidéo pour filmer leurs répétitions, le plus souvent dans le but de créer une « mémoire » de la compagnie, d’enregistrer ces moments fugaces et souvent décrits comme « magiques » que sont les répétitions, force est de constater que ces heures de captations sont rarement « traitées » et s’entassaient hier dans des cartons (en format dv) ou s’accumulent aujourd’hui sur des disques durs externes.

%Reprenant un dispositif qui avait déjà été expérimenté au cours d’un projet précédent, Spectacle en ligne (3), nous avons placé une unique caméra au milieu de l’orchestre, une position qui est également privilégiée par le metteur en scène pour observer les répétitions. Nous avons suivi en cela une proposition ingénieuse de Jean-Luc Godard (4) : « Pourquoi les gens de théâtre n’ont-ils jamais envie de filmer leurs spectacles pour les garder comme archives ? (…) Ce serait très simple : la caméra au milieu de l’orchestre avec un objectif moyen – mais pas le zoom, qui donnerait déjà lieu à une interprétation ».

%Ce « point de vue du metteur en scène » présente plusieurs avantages théoriques et pratiques. D’une part, c’est le point de vue le plus adapté à la projection des films des spectacles dans la même salle. D’autre part, c’est le point de vue le plus proche des acteurs, et le seul qui permette de saisir le jeu des regards entre les acteurs et la salle. Enfin, c’est également le point de vue pour lequel les éclairages sont mis au point, ce qui nous permet de filmer sans modifier ces éclairages. Ce dernier point reste difficile à réaliser en pratique, surtout lorsque les éclairages varient brusquement, mais cela nous paraît important de respecter les choix de mise en scène, ce qui n’est possible que de ce seul point de vue.

%Comme le souligne justement Pascal Bouchez (5), une problématique particulière à la captation vidéo, c’est l’opposition entre le traitement parallèle de l’information au théâtre (le spectateur voit l’ensemble des acteurs et perçoit globalement la scène), et le traitement séquentiel de cette même information au cinéma ou à la télévision (le spectateur ne voit que les acteurs choisis par le réalisateur et perçoit donc de façon séquentielle la scène à travers une suite d’images). Ainsi, le suivi séquentiel des dialogues peut être problématique lorsque ceux-ci font intervenir trois acteurs éloignés. Un plan fixe des trois acteurs ne permet pas facilement au spectateur de se repérer à l’écran comme il le ferait face à la scène. Une série de gros plans peut être utilisée pour diriger l’attention du spectateur. Il faut donc bien comprendre le système cognitif de l’attention et son fonctionnement dans les deux situations différentes de la scène et de l’écran.

%Les techniques classiques du cinéma permettent en principe de résoudre ces différents problèmes, par une transposition entre les langages dramatique et cinématographique. Mais dans les conditions du direct, le réalisateur est de plus en plus démuni au fur et à mesure que croît le volume spatial de la scène. Comme l’écrit Pascal Bouchez, “tout se joue en direct, si vite que les plans dont la création nécessiteraient de nombreuses répétitions et une longue préparation au cinéma – sont impossibles au théâtre”.

 %Le projet de recherche Kino Ai aborde précisément cette question grâce à des techniques d’intelligence artificielle qui proposent automatiquement des solutions de cadrage et de montage montrant les actions scéniques et leur enchainement : les données extraites des heures filmées peuvent ainsi s’adapter aux besoins exprimés soit par les professionnels du spectacle, soit par les enseignants et les chercheurs (archivage pour la compagnie, communication auprès des diffuseurs, documentation pour la pédagogie et/ou la recherche).

%On peut remarquer que cette méthode de recadrage en post-production est une option technique et artistique nouvelle, décrite par Walter Murch sous le nom de montage vertical (6), et qui permet de contrôler le « zoom de l’interprétation » dont parlait Jean-Luc Godard en post-production. Cette technique est particulière fastidieuse pour les monteurs, mais se prête en revanche très bien au traitement informatique.

%A partir d’une captation unique, nous proposons ainsi des solutions de montage multiples, destinés à visualiser la captation selon plusieurs lectures possibles. Notre approche tire parti du fait que tous les rushes peuvent être virtuellement disponibles. Dans un autre contexte, Francis Ford Coppola a utilisé cette possibilité pour intervenir en direct sur le montage de son film Twixt lors de projections en festivals (7).

%En suivant ce principe, nous calculons plusieurs cadres mettant en avant les différents aspects de la représentation théâtrale : décors et mouvements d’acteurs en plan large ; codes de proximités entre les acteurs en plan moyen ; langage verbal et non verbal en plan rapproché. Chaque série de plans ainsi recadrés peut être organisée en temps réel en un montage dédié au point de vue choisi. Cette technique permet l’exploration de la représentation sous ses différents aspects.

%-----------------------------------------
\section{State of the art}
Previous work in intelligent cinematography and editing is numerous.

Some previous work has been devoted to generating cinematographic rushes from wide-screen video in various contexts, including meetings \cite{???}, courses \cite{???}, video conferences \cite{???} and live performances \cite{Gandhi2014,Kumar2017}.


The problem of creating a multi-view edited video from limited
input camera views has been considered previously in very specialized
scenarios. The Virtual Videography system \cite{Heck2007} used virtual
PTZ to simulate multiple cameras from a lecture video. The
MSLRCS \cite{Zhang2005} and AutoAuditorium \cite{Bianchi2004} systems 
use a small set of fixed views including input of presentation slides. These systems achieve full automation, albeit at the expense of allowing for creativity
and human input in the editing process. They are also limited
to working in the more constrained environment of usually a
single presenter in front of a chalkboard or a slide screen. Extending
to the richer environment of multiple actors in more complex
stagings would be challenging, especially as it requires a richer set
of shot types to be generated. In contrast, our system addresses
only the rush generation aspect, but can generate a rich range of
shot types from more complex scenarios including multiple actors.

Remarkably little work as been devoted specifically to the problem
of optimizing the composition of a virtual PTZ camera in postproduction.
Recent work has focused more on providing interactive
control of the virtual PTZ camera in real time \cite{Gaddam2014a,Gaddam2014b}. A method for automatic editing of basketball games was also proposed
by Carr et al. \cite{Carr2013} employing both robotic and virtual PTZ cameras.
The robotic camera follows the centroid of the detected players and
then a virtual camera is employed to crop subregions of the obtained
images to compensate for motor errors. Because they are
targeting online applications, their method makes decisions in near
real time (with a small delay), which can lead to sub-optimal solutions.
To the best of our knowledge, our technique provides the first
general solution to the problem for offline computation of a virtual
pan-tilt-zoom camera shot given a list of visual targets over the entire
duration of a recorded performance.

The question of a computational model to describe “good” camera
movements, particularly in terms of subwindows of video, has been
considered by work in video stabilization. While most previous work in
video stablization simply aim to remove jitter, Re-Cinematography
\cite{Gleicher2008} formalized cinematic principles in terms of movement in the
frame for computation. Grundmann et al. then showed that this
can be formulated in an optimization framework \cite{Grundmann2011}. We build on this computational formulation of camera movement, extending it to the
problem of multiple rush generation.

Several frameworks for automatically cropping sub-clips from a
panoramic video and editing them together into a movie in realtime
has been proposed for the case of sports events \cite{Daniyal2011,Schreer2013}. Operating in real-time limits the capability of that system to tracking of
simple targets. Because we are focusing on post-production, rather
than live broadcast, we are able to perform tracking and recognition
of multiple actors even in complex cases, which makes our method
more generally applicable to rich cultural heritage content. Furthermore,
our method can be used to generate arbitrary shot compositions.

Pano2Vid \cite{Su2016} is a new computer vision problem where the task is to  automatically control the pose and motion of a virtual normal-field-of-view (NFOV) camera within an input 360° video. Camera control must be optimized to produce video that could conceivably have been captured by a human observer equipped with a real NFOV camera. 

Using computer vision to control cameras and create full-edited
movies is not a new idea. Pinhanez and Bobick \cite{Pinhanez1997} have investigated the use of low-level motion tracking to control TV cameras  but their method is limited to closed-world domains (exemplified
by cooking shows) and requires extensive domain-specific
knowledge. 

Our method assumes a pre-processing stage, where actors are tracked
and the location of their heads and floor projections are recovered
in each frame of the input video. We use actor poses detected by the OpenPose software as an input \cite{OpenPose}. Kinoai includes software for automatically linking those poses into tracklets  and a graphical user interface for labeling and naming tracklets. 
 
\RR{Include more references for tracking and naming actors}

\RR{Include more references for cropping panoramic video}



Tedial  proposes a technology called SmartLive For Live Events And Production
\footnote{Tedial behind the play, 2019, \url{https://www.tedial.com}}.

Pixellot’s [4] patented technology streamlines the production workflow by deploying an unmanned multi-camera system in a single fixed rig \footnote{Pixellot Automatic Production,» 2019 \url{https://www.pixellot.tv}}.

Seervision \footnote{\url{https://www.seervision.com}} has analysed the motion sequences of cameramen in various scenarios and converted them into video analysis algorithms for real-time object recognition and scene segmentation. 


Other previous  work has investigated automatic film editing of multi-camera live performances\cite{Wright2018} and dialogue scenes \cite{Leake2017}.

Automated video capture and analysis of live theatre was the focus of the "spectacle en ligne(s)" experimental system, which was used to create an online dataset of 300 hours of rehearsals \cite{Ronfard2015}. 

To the best of our knowledge, there is no existing  open source programming environment for consolidating this preview work together. Kino AI aims to provide such an environment. 

